On Solving the Rubik's Cube with Domain-Independent Planners Using Standard Representations

Rubik's Cube (RC) is a well-known and computationally challenging puzzle that has motivated AI researchers to explore efficient alternative representations and problem-solving methods. The ideal situation for planning here is that a problem be solved optimally and efficiently represented in a standard notation using a general-purpose solver and heuristics. The fastest solver today for RC is DeepCubeA with a custom representation, and another approach is with Scorpion planner with State-Action-Space+ (SAS+) representation. In this paper, we present the first RC representation in the popular PDDL language so that the domain becomes more accessible to PDDL planners, competitions, and knowledge engineering tools, and is more human-readable. We then bridge across existing approaches and compare performance. We find that in one comparable experiment, DeepCubeA (trained with 12 RC actions) solves all problems with varying complexities, albeit only 78.5% are optimal plans. For the same problem set, Scorpion with SAS+ representation and pattern database heuristics solves 61.50% problems optimally, while FastDownward with PDDL representation and FF heuristic solves 56.50% problems, out of which 79.64% of the plans generated were optimal. Our study provides valuable insights into the trade-offs between representational choice and plan optimality that can help researchers design future strategies for challenging domains combining general-purpose solving methods (planning, reinforcement learning), heuristics, and representations (standard or custom).

==> content/algotexs/HDDL.tex <==
% This file is part of https://github.com/Maumagnaguagno/Planning_LaTeX
\lstdefinelanguage{HDDL}
{
  sensitive=false,    % not case-sensitive
  morecomment=[l]{;}, % line comment
  alsoletter={:,-},   % consider extra characters
  morekeywords={
    define,domain,problem,not,and,or,forall,exists,
    :domain,:requirements,:typing,:hierarchy,:equality,:negative-preconditions,
    :method-preconditions,:universal-preconditions,:universal-effects,:existential-preconditions,
    :types,:predicates,:action,:parameters,:precondition,:effect,
    :task,:method,:subtasks,:tasks,:ordered-subtasks,:ordered-tasks,:ordering,:constraints,
    :htn,:init,:goal,:objects
  }
}

==> content/algotexs/JSHOP.tex <==
% This file is part of https://github.com/Maumagnaguagno/Planning_LaTeX
\lstdefinelanguage{JSHOP}
{
  sensitive=false,    % not case-sensitive
  morecomment=[l]{;}, % line comment
  alsoletter={:,-},   % consider extra characters
  morekeywords={
    defdomain,defproblem,not,and,or,imply,forall,assign,call,nil,
    :first,:sort-by,:immediate,:unordered,:operator,:method,:protection,:-
  }
}

==> content/system.tex <==
\section{System Description}

%In this section, we define 
We now  discuss how an RC can be modelled in PDDL and how the generated plan is linked with a visualizer for providing better understanding to people coming from a non-planning background as well. 

% \begin{figure}[!b]
%  \centering
%  \includegraphics[scale=0.3]{content/images/rubiks_cube.png}
%  \caption{Rubik's cube description to define the domain encoding.}
%  \label{FIG: rubiks-cube}
% \end{figure}

% \begin{figure}[tb]
%  \centering
%  \includegraphics[scale=0.37]{content/images/rubiks_action.png}
%  \caption{Action {\em D} in Rubik's cube problem.}
%  \label{FIG: rubiks-action}
% \end{figure}

% \begin{algorithm}[tb]
% \caption{For Action D (Down)}
% \label{alg:action_d}
% \begin{algorithmic}[1] %[1] enables line numbers
% \FOR{cubelet in corner cubes of D layer}
% \FORALL{?x ?y ?z}
% \STATE not cubelet(x,y,z)
% \STATE assign right-adjacent-cubelet(y,x,z) 
% \ENDFOR
% \ENDFOR
% \FOR{edge-cube in edge cubes of D layer}
% \FORALL{?a ?z}
% \STATE not edge-cube(a,z)
% \STATE assign right-adjacent-edge-cube(a,z) 
% \ENDFOR
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

% \subsection{Generating and Visualizing the Plan}



==> content/visualization.tex <==
\section{Visualization for Plan Validity}
Our system's PDDL encoded RC solver, in combination with a Visualizer, generates plan actions to solve the problem using the Fast-Downward (FD) AI planner. We have used publicly available Tkinter based Visualizer code\footnote{\url{https://code-projects.org/rubiks-cube-in-python-with-source-code/}} for plan visualization. A random scrambled state of RC represented in the Visualizer is shown in the Figure \ref{FIG: shuffled-cube}. AI planners are controllable in generating the desired plans. We can specify the search algorithm and the heuristics to the Fast-Downward planner. Each different search algorithm generates different plans to reach the goal state. We employed A\textsuperscript{*} search algorithm in combination with landmark-count heuristics which supports conditional-effects in our system and gives plans in minutes.

The system architecture is shown in Figure \ref{FIG: system}. For diverse types of audiences, our solution offers two main features:
% \noindent (a) 
% \begin{enumerate}[label=(\alph*)]
%     \item 
    (a) By giving the Fast-Downward planner path together with the problem file holding the cube's initial scrambled state, the system may be used to solve any RC problem. It creates an actions plan file as a solution for the problem file given and then launches the Visualizer. The user may visually follow the actions in the plan file generated to observe the RC being solved step by step.
    %\item 
    %\noindent 
    (b) The visualizer may also be used by a user with their own problem file and actions plan file to see the RC being solved step by step from the actions in the plan file. This will assist the user in comprehending the many states being explored in order to arrive at the solved goal state from the initial state set by the user.
%&\end{enumerate}

% \begin{figure}[!t]
%  \centering
%  \includegraphics[scale = 0.17]{content/images/shuffled_cube_new.png}
%  \caption{Shuffled state of the cube. Solution found with FD planner: U, L. Cost: 2.}
%  \label{FIG: shuffled-cube}
% \end{figure}

% \begin{figure}[!t]
%  \centering
%  \includegraphics[scale=0.30]{content/images/system.png}
%  \caption{System architecture: input  path 1 or 2 is needed.}
%  \label{FIG: system}
% \end{figure}
% \vspace{-0.1in}
